Calibration and Correctness of Language Models for Code

Machine learning models are widely used, but can also often be wrong. Users would benefit from a reliable indication of whether a given output from a given model should be trusted, so a rational decision can be made whether to use the output or not. For example, outputs can be associated with a confidence measure; if this confidence measure is strongly associated with likelihood of correctness, then the model is said to be well-calibrated. A well-calibrated confidence measure can serve as a basis for rational, graduated decision-making on how much review and care is needed when using generated code. Calibration has so far been studied in mostly non-generative (e.g. classification) settings, especially in software engineering. However, generated code can quite often be wrong: Given generated code, developers must decide whether to use directly, use after varying intensity of careful review, or discard model-generated code. Thus, calibration is vital in generative settings. We make several contributions. We develop a framework for evaluating the calibration of code-generating models. We consider several tasks, correctness criteria, datasets, and approaches, and find that, by and large, generative code models we test are not well-calibrated out of the box. We then show how calibration can be improved using standard methods, such as Platt scaling. Since Platt scaling relies on the prior availability of correctness data, we evaluate the applicability and generalizability of Platt scaling in software engineering, discuss settings where it has good potential for practical use, and settings where it does not. Our contributions will lead to better-calibrated decision-making in the current use of code generated by language models, and offers a framework for future research to further improve calibration methods for generative models in software engineering.

==> authors_acm.tex <==
\author{Claudio Spiess}
\authornote{Both first authors contributed equally to this research. Order determined by random coin flip.}
\orcid{0009-0000-5932-7022}
\email{cvspiess@ucdavis.edu}
\affiliation{
    \institution{UC Davis}
    \country{USA}
}

\author{David Gros}
\authornotemark[1]
\orcid{0009-0001-4212-2204}
\email{dgros@ucdavis.edu}
\affiliation{
    \institution{UC Davis}
    \country{USA}
}

\author{Kunal Suresh Pai}
\orcid{0009-0003-0675-7135}
\affiliation{
    \institution{UC Davis}
    \country{USA}
}
\email{kunpai@ucdavis.edu}

\author{Michael Pradel}
\orcid{0000-0003-1623-498X}
\affiliation{
    \institution{Univ. of Stuttgart}
    \country{Germany}
}
\email{michael@binaervarianz.de}

\author{Md Rafiqul Islam Rabin}
\orcid{0000-0001-5575-0528}
\affiliation{
    \institution{Univ. of Houston}
    \country{USA}
}
\email{mrabin@central.uh.edu}

\author{Amin Alipour}
\orcid{0000-0002-6479-7202}
\affiliation{
    \institution{Univ. of Houston}
    \country{USA}
}
\email{maalipou@central.uh.edu}

\author{Susmit Jha}
\orcid{0000-0001-5983-9095}
\affiliation{
    \institution{SRI}
    \country{USA}
}
\email{susmit.jha@sri.com}

\author{Prem Devanbu}
\orcid{0000-0002-4346-5276}
\affiliation{
    \institution{UC Davis}
    \country{USA}
}
\email{ptdevanbu@ucdavis.edu}

\author{Toufique Ahmed}
\orcid{0000-0002-4427-1350}
\affiliation{
    \institution{UC Davis}
    \country{USA}
}
\email{tfahmed@ucdavis.edu}

==> tables/correctness.tex <==
\definecolor{improvement}{rgb}{1,0,0}
\definecolor{modelrow}{gray}{0.85}

\begin{table}{r}{7.5cm}
	\centering
	\resizebox{7.5cm}{!}{
		\begin{tblr}{
				colspec = {lcccc},
				vline{4} = {3-7}{gray!75,dotted},
				columns = {font=\small},
			}

			                           & \SetCell[c=2]{c} All Pass@1 &                & \SetCell[c=2]{c} Exact-Match         &                \\
			\cmidrule[lr,gray!75]{2-3} & Docstring                   & No Docstring   & \cmidrule[lr,gray!75]{4-5} Docstring & No Docstring   \\

			\midrule

			CodeGen2                   & 28.84                       & 23.10          & 19.68                                & 15.10          \\
			Codex                      & 32.96                       & 21.69          & 23.60                                & 17.77          \\
			GPT-3.5                    & \textbf{33.22}              & \textbf{26.77} & \textbf{23.96}                       & \textbf{18.72} \\
			\bottomrule
		\end{tblr}
	}
	\caption{\scriptsize Performance comparison of models on DyPyBench Line Completion task: experiments include With and Without Docstring. Metrics are All Pass at Rank 1 (\textbf{All Pass@1}), meaning all project test cases passed with the line completion on first and only sample (at $t=0$), and Exact-Match, meaning the line completion was an exact string match with the original project line. Boldface signifies high performing model for dataset and metric.}
	\label{fig:modelPerformanceComparison}
\end{table}

==> tables/dypybench_test_exact_confusion.tex <==
\begin{table}[!ht]
	\centering
	%\resizebox{0.97\columnwidth}{!}{
	\begin{tabular}{lrrr}
		\toprule
		                     & \multicolumn{2}{c}{All Pass@1} &                                \\ % Adjusted for clarity
		\textbf{Exact-Match} & \textbf{False}                 & \textbf{True} & \textbf{Total} \\
		\midrule
		False                & 59.89\%                        & 16.16\%       & 76.04\%        \\
		True                 & 6.89\%                         & 17.06\%       & 23.96\%        \\
		Total                & 66.78\%                        & 33.22\%       & 100.00\%       \\
		\bottomrule
	\end{tabular}
	%}
	\caption{\scriptsize Matrix of all tests passed versus exact-match notions of correctness for DyPyBench (with Docstring). Metrics are All Pass at Rank 1 (\textbf{All Pass@1}), meaning all project test cases passed with the line completion on first and only sample (at $t=0$), and Exact-Match, meaning the line completion was an exact string match with the original project line.}
	\label{tab:mainDyPyCorrectnessMatrix}
	% \vspace{-0.15in} % Adjust or remove as needed based on your document's spacing requirements
\end{table}

==> tables/generated_tables/brierAllPassedRaw_baksub.tex <==
% This file was autogenerated by gen_table.py
% SHA 27cfcbd282 - UNCOMMITED CHANGES
% Generate Date UTC 2024-01-23-05-56-27
% It is not recommended to edit this file directly
\definecolor{improvement}{rgb}{1,0,0}
\definecolor{modelrow}{gray}{0.85}

\begin{table*}
    \centering
    \resizebox{0.8\textwidth}{!}{
        \begin{tblr}{
            colspec = {llccccccccccccccc},
            vline{3,6,9,12,15} = {4-24}{gray!75, dotted},
            columns = {font=\small},
                }
            &  & \SetCell[c=3]{c} \textbf{Line Completion} & & & \SetCell[c=6]{c} \textbf{Function Synthesis} & & & & & & \SetCell[c=6]{c} \textbf{Program Repair} & & & & &  \\

            \cmidrule[gray!75]{3-6} \cmidrule[lr,gray!75]{6-11} \cmidrule[l,gray!75]{12-17}
             & & \SetCell[c=3]{c} DyPyBench & & & \SetCell[c=3]{c} HumanEval & & & \SetCell[c=3]{c} MBPP & & & \SetCell[c=3]{c} Defects4J & & & \SetCell[c=3]{c} SStubs \\
            \cmidrule[lr]{3-5} \cmidrule[lr]{6-8} \cmidrule[lr]{9-11} \cmidrule[lr]{12-14} \cmidrule[l]{15-17}
            Model & Metric & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ \\
            \cmidrule[l]{1-17}
GPT-3.5
    & Total Prob
        & \textbf{0.23} & \textbf{-0.03} & 0.15
        & 0.62 & -1.70 & 0.63
        & 0.71 & -2.50 & 0.71
        & 0.25 & -0.63 & 0.28
        & 0.24 & -0.50 & 0.25
    \\
    & Avg Prob
        & 0.41 & -0.87 & 0.46
        & 0.27 & -0.18 & 0.23
        & \textbf{0.22} & \textbf{-0.09} & \textbf{0.14}
        & 0.68 & -3.39 & 0.73
        & 0.64 & -2.94 & 0.69
    \\
    & Ask T/F
        & 0.25 & -0.13 & 0.16
        & 0.34 & -0.47 & 0.37
        & 0.33 & -0.64 & 0.38
        & \textbf{0.15} & \textbf{+0.05} & \textbf{0.04}
        & \textbf{0.16} & \textbf{-0.01} & \textbf{0.04}
    \\
    & Ask T/F N
        & 0.25 & -0.15 & \textbf{0.15}
        & \textbf{0.23} & \textbf{+0.01} & 0.19
        & 0.22 & -0.11 & 0.16
        & 0.20 & -0.30 & 0.24
        & 0.22 & -0.34 & 0.23
    \\
    & Verbalize
        & 0.43 & -0.92 & 0.42
        & 0.28 & -0.24 & 0.22
        & 0.24 & -0.17 & 0.17
        & 0.58 & -2.72 & 0.60
        & 0.50 & -2.09 & 0.53
    \\
    & Length
        & 0.44 & -0.99 & 0.46
        & 0.23 & -0.03 & \textbf{0.15}
        & 0.22 & -0.10 & 0.16
        & 0.53 & -2.43 & 0.60
        & 0.53 & -2.26 & 0.60
    \\
    & Unskilled
        & 0.22 &  0.00 & 0.00
        & 0.23 &  0.00 & 0.00
        & 0.20 &  0.00 & 0.00
        & 0.15 &  0.00 & 0.00
        & 0.16 &  0.00 & 0.00
    \\
\hline[dashed]
Codex
    & Total Prob
        & \textbf{0.23} & \textbf{-0.02} & 0.16
        & 0.44 & -0.77 & 0.45
        & 0.60 & -1.52 & 0.60
        & 0.25 & -0.39 & 0.24
        & 0.20 &  0.00 & 0.09
    \\
    & Avg Prob
        & 0.46 & -1.07 & 0.50
        & 0.34 & -0.38 & 0.35
        & \textbf{0.24} & \textbf{-0.03} & \textbf{0.19}
        & 0.66 & -2.68 & 0.69
        & 0.58 & -1.90 & 0.62
    \\
    & Ask T/F
        & 0.24 & -0.09 & 0.12
        & 0.37 & -0.47 & 0.36
        & 0.49 & -1.06 & 0.50
        & \textbf{0.18} & \textbf{+0.01} & \textbf{0.07}
        & \textbf{0.19} & \textbf{+0.03} & \textbf{0.02}
    \\
    & Ask T/F N
        & 0.23 & -0.06 & \textbf{0.07}
        & \textbf{0.32} & \textbf{-0.29} & \textbf{0.30}
        & 0.42 & -0.79 & 0.43
        & 0.25 & -0.41 & 0.27
        & 0.23 & -0.14 & 0.18
    \\
    & Verbalize
        & 0.38 & -0.74 & 0.35
        & 0.42 & -0.67 & 0.40
        & 0.38 & -0.61 & 0.33
        & 0.47 & -1.65 & 0.50
        & 0.43 & -1.14 & 0.42
    \\
    & Length
        & 0.43 & -0.95 & 0.45
        & 0.44 & -0.77 & 0.44
        & 0.56 & -1.35 & 0.56
        & 0.50 & -1.79 & 0.55
        & 0.56 & -1.78 & 0.59
    \\
    & Unskilled
        & 0.22 &  0.00 & 0.00
        & 0.25 &  0.00 & 0.00
        & 0.24 &  0.00 & 0.00
        & 0.18 &  0.00 & 0.00
        & 0.20 &  0.00 & 0.00
    \\
\hline[dashed]
CodeGen2
    & Total Prob
        & \textbf{0.21} & \textbf{-0.02} & 0.15
        & \textbf{0.23} & \textbf{-0.30} & \textbf{0.23}
        & 0.29 & -0.41 & 0.29
        & - & - & -
        & - & - & -
    \\
    & Avg Prob
        & 0.44 & -1.16 & 0.50
        & 0.60 & -2.39 & 0.66
        & 0.58 & -1.80 & 0.61
        & - & - & -
        & - & - & -
    \\
    & Ask T/F
        & 0.23 & -0.10 & \textbf{0.14}
        & 0.25 & -0.38 & 0.24
        & \textbf{0.25} & \textbf{-0.19} & \textbf{0.21}
        & - & - & -
        & - & - & -
    \\
    & Ask T/F N
        & 0.33 & -0.59 & 0.35
        & 0.39 & -1.19 & 0.45
        & 0.39 & -0.88 & 0.43
        & - & - & -
        & - & - & -
    \\
    & Verbalize
        & 0.42 & -1.04 & 0.41
        & 0.43 & -1.39 & 0.42
        & 0.40 & -0.94 & 0.38
        & - & - & -
        & - & - & -
    \\
    & Length
        & 0.47 & -1.28 & 0.51
        & 0.38 & -1.14 & 0.42
        & 0.33 & -0.58 & 0.28
        & - & - & -
        & - & - & -
    \\
    & Unskilled
        & 0.21 &  0.00 & 0.00
        & 0.18 &  0.00 & 0.00
        & 0.21 &  0.00 & 0.00
        & - & - & -
        & - & - & -
    \\
\bottomrule
        \end{tblr}
    }
         \caption{\scriptsize Calibration measured as raw, non-scaled Brier Score (${\mathcal B}$, $\downarrow$ lower better), Skill Score ($SS$, $\uparrow$ higher better), and Expected Calibration Error ($ECE$, $\downarrow$ lower better), with respect to ``all passed'' notion of correctness, except SStubs which is ``exact-match''. CodeGen2 repair values are omitted as it does not perform the task with greater than 1\% accuracy. The ``Unskilled" row corresponds to a naive approach where the confidence is always returned as the base correctness rate, with Skill Score ($SS$) always zero by definition.}
         \label{tab:brierAllPassedRaw}
     \vspace*{-1\baselineskip}
\end{table*}

==> tables/generated_tables/brierAllPassedScaled_baksub.tex <==
% This file was autogenerated by gen_table.py
% SHA 27cfcbd282 - UNCOMMITED CHANGES
% Generate Date UTC 2024-01-23-05-56-28
% It is not recommended to edit this file directly
\definecolor{improvement}{rgb}{1,0,0}
\definecolor{modelrow}{gray}{0.85}

\begin{table*}
    \centering
    \resizebox{0.8\textwidth}{!}{
        \begin{tblr}{
            colspec = {llccccccccccccccc},
            vline{3,6,9,12,15} = {4-24}{gray!75, dotted},
            columns = {font=\small},
                }
            &  & \SetCell[c=3]{c} \textbf{Line Completion} & & & \SetCell[c=6]{c} \textbf{Function Synthesis} & & & & & & \SetCell[c=6]{c} \textbf{Program Repair} & & & & &  \\

            \cmidrule[gray!75]{3-6} \cmidrule[lr,gray!75]{6-11} \cmidrule[l,gray!75]{12-17}
             & & \SetCell[c=3]{c} DyPyBench & & & \SetCell[c=3]{c} HumanEval & & & \SetCell[c=3]{c} MBPP & & & \SetCell[c=3]{c} Defects4J & & & \SetCell[c=3]{c} SStubs \\
            \cmidrule[lr]{3-5} \cmidrule[lr]{6-8} \cmidrule[lr]{9-11} \cmidrule[lr]{12-14} \cmidrule[l]{15-17}
            Model & Metric & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ \\
            \cmidrule[l]{1-17}
GPT-3.5
    & Total Prob
        & 0.21 & +0.07 & 0.03
        & \textbf{0.20} & \textbf{+0.15} & 0.09
        & 0.19 & +0.07 & 0.05
        & 0.16 & -0.05 &
        & \textbf{0.16} & \textbf{+0.03} &
    \\
    & Avg Prob
        & \textbf{0.20} & \textbf{+0.08} & 0.04
        & 0.23 & -0.02 &
        & 0.20 &  0.00 &
        & 0.16 & -0.03 &
        & 0.16 & +0.02 &
    \\
    & Ask T/F
        & 0.22 &  0.00 &
        & 0.20 & +0.12 & 0.11
        & 0.18 & +0.09 & 0.06
        & \textbf{0.15} & \textbf{+0.05} &
        & 0.16 &  0.00 &
    \\
    & Ask T/F N
        & 0.22 &  0.00 &
        & 0.20 & +0.14 & 0.07
        & \textbf{0.18} & \textbf{+0.11} & 0.04
        & 0.15 & +0.04 &
        & 0.16 & +0.01 &
    \\
    & Verbalize
        & 0.22 &  0.00 &
        & 0.24 & -0.05 &
        & 0.20 & +0.02 &
        & 0.17 & -0.09 &
        & 0.16 &  0.00 &
    \\
    & Length
        & 0.22 &  0.00 &
        & 0.24 & -0.03 &
        & 0.20 & +0.01 &
        & 0.16 & -0.06 &
        & 0.16 &  0.00 &
    \\
    & Unskilled
        & 0.22 &  0.00 &
        & 0.23 &  0.00 &
        & 0.20 &  0.00 &
        & 0.16 &  0.00 &
        & 0.16 &  0.00 &
    \\
\hline[dashed]
Codex
    & Total Prob
        & \textbf{0.20} & \textbf{+0.09} & 0.03
        & 0.22 & +0.11 & 0.08
        & 0.22 & +0.06 & 0.04
        & 0.18 & -0.01 &
        & \textbf{0.19} & \textbf{+0.05} & 0.02
    \\
    & Avg Prob
        & 0.20 & +0.09 & 0.04
        & \textbf{0.22} & \textbf{+0.14} & 0.07
        & \textbf{0.21} & \textbf{+0.12} & 0.06
        & 0.18 & -0.02 &
        & 0.19 & +0.05 & 0.02
    \\
    & Ask T/F
        & 0.22 &  0.00 &
        & 0.24 & +0.03 &
        & 0.24 &  0.00 &
        & 0.18 &  0.00 &
        & 0.19 & +0.04 &
    \\
    & Ask T/F N
        & 0.22 &  0.00 &
        & 0.24 & +0.03 &
        & 0.24 &  0.00 &
        & 0.18 & -0.01 &
        & 0.20 & +0.02 &
    \\
    & Verbalize
        & 0.22 &  0.00 &
        & 0.26 & -0.02 &
        & 0.24 & -0.01 &
        & \textbf{0.18} & \textbf{ 0.00} &
        & 0.20 &  0.00 &
    \\
    & Length
        & 0.22 & +0.01 &
        & 0.26 & -0.03 &
        & 0.24 & -0.01 &
        & 0.20 & -0.10 &
        & 0.20 &  0.00 &
    \\
    & Unskilled
        & 0.22 &  0.00 &
        & 0.25 &  0.00 &
        & 0.24 &  0.00 &
        & 0.18 &  0.00 &
        & 0.20 &  0.00 &
    \\
\hline[dashed]
CodeGen2
    & Total Prob
        & \textbf{0.19} & \textbf{+0.08} & 0.04
        & 0.18 &  0.00 &
        & 0.21 &  0.00 &
        & - & - &
        & - & - &
    \\
    & Avg Prob
        & 0.19 & +0.07 & 0.02
        & 0.17 & +0.03 &
        & 0.21 &  0.00 &
        & - & - &
        & - & - &
    \\
    & Ask T/F
        & 0.21 &  0.00 &
        & 0.18 & -0.01 &
        & \textbf{0.20} & \textbf{+0.01} &
        & - & - &
        & - & - &
    \\
    & Ask T/F N
        & 0.21 &  0.00 &
        & \textbf{0.17} & \textbf{+0.04} &
        & 0.21 &  0.00 &
        & - & - &
        & - & - &
    \\
    & Verbalize
        & 0.21 &  0.00 &
        & 0.18 & -0.01 &
        & 0.21 &  0.00 &
        & - & - &
        & - & - &
    \\
    & Length
        & 0.21 &  0.00 &
        & 0.18 & -0.02 &
        & 0.21 &  0.00 &
        & - & - &
        & - & - &
    \\
    & Unskilled
        & 0.21 &  0.00 &
        & 0.18 &  0.00 &
        & 0.21 &  0.00 &
        & - & - &
        & - & - &
    \\
\bottomrule
        \end{tblr}
    }
         \caption{\scriptsize Calibration measured as Platt-scaled Brier Score (${\mathcal B}$, $\downarrow$ lower better), Skill Score ($SS$, $\uparrow$ higher better), and Expected Calibration Error ($ECE$, $\downarrow$ lower better), with respect to ``all passed'' notion of correctness, except SStubs which is ``exact-match''. In cases where the $SS$ is less than 0.05, the $ECE$ is omitted. This is because an estimate without any signal will become Platt-scaled to approximately the base rate. This will \emph{appear} as one well calibrated bin, resulting in an $ECE$ near zero, but does not provide information. CodeGen2 repair values are omitted as it does not perform the task with greater than 1\% accuracy.}
         \label{tab:brierAllPassedScaled}
     \vspace*{-1\baselineskip}
\end{table*}

==> tables/generated_tables/brierExactMatchRaw.tex <==
% This file was autogenerated by gen_table.py
% SHA 27cfcbd282 - UNCOMMITED CHANGES
% Generate Date UTC 2024-01-23-05-56-30
% It is not recommended to edit this file directly
\definecolor{improvement}{rgb}{1,0,0}
\definecolor{modelrow}{gray}{0.85}

\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tblr}{
            colspec = {llccccccccc},
            vline{3,6,9} = {4-24}{gray!75, dotted},
            columns = {font=\small},
                }
            &  & \SetCell[c=3]{c} \textbf{Line Completion} & & & \SetCell[c=6]{c} \textbf{Program Repair} & & & & &  \\

            \cmidrule[gray!75]{3-6} \cmidrule[lr,gray!75]{6-11}
             & & \SetCell[c=3]{c} DyPyBench & & & \SetCell[c=3]{c} Defects4J & & & \SetCell[c=3]{c} SStubs \\
            \cmidrule[lr]{3-5} \cmidrule[lr]{6-8} \cmidrule[lr]{9-11}
            Model & Metric & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ & ${\mathcal B}$ & $SS$ & $ECE$ \\
            \hline
GPT-3.5
    & Total Prob
        & \textbf{0.11} & \textbf{+0.38} & \textbf{0.03}
        & 0.23 & -0.77 & 0.28
        & 0.24 & -0.50 & 0.25
    \\
    & Avg Prob
        & 0.45 & -1.46 & 0.55
        & 0.71 & -4.57 & 0.77
        & 0.64 & -2.94 & 0.69
    \\
    & Ask T/F
        & 0.20 & -0.10 & 0.12
        & \textbf{0.13} & \textbf{+0.02} & \textbf{0.07}
        & \textbf{0.16} & \textbf{-0.01} & \textbf{0.04}
    \\
    & Ask T/F N
        & 0.24 & -0.29 & 0.17
        & 0.19 & -0.53 & 0.27
        & 0.22 & -0.34 & 0.23
    \\
    & Verbalize
        & 0.47 & -1.58 & 0.50
        & 0.58 & -3.55 & 0.62
        & 0.50 & -2.09 & 0.53
    \\
    & Length
        & 0.48 & -1.62 & 0.55
        & 0.55 & -3.34 & 0.64
        & 0.53 & -2.26 & 0.60
    \\
    & Unskilled
        & 0.18 &  0.00 & 0.00
        & 0.13 &  0.00 & 0.00
        & 0.16 &  0.00 & 0.00
    \\
\hline[dashed]
Codex
    & Total Prob
        & \textbf{0.10} & \textbf{+0.43} & \textbf{0.02}
        & 0.23 & -0.46 & 0.23
        & 0.20 &  0.00 & 0.09
    \\
    & Avg Prob
        & 0.51 & -1.80 & 0.60
        & 0.69 & -3.47 & 0.74
        & 0.58 & -1.90 & 0.62
    \\
    & Ask T/F
        & 0.19 & -0.07 & 0.10
        & \textbf{0.16} & \textbf{-0.04} & \textbf{0.12}
        & \textbf{0.19} & \textbf{+0.03} & \textbf{0.02}
    \\
    & Ask T/F N
        & 0.21 & -0.17 & 0.12
        & 0.25 & -0.63 & 0.31
        & 0.23 & -0.14 & 0.18
    \\
    & Verbalize
        & 0.40 & -1.20 & 0.41
        & 0.46 & -1.96 & 0.50
        & 0.43 & -1.14 & 0.42
    \\
    & Length
        & 0.47 & -1.59 & 0.54
        & 0.52 & -2.36 & 0.59
        & 0.56 & -1.78 & 0.59
    \\
    & Unskilled
        & 0.18 &  0.00 & 0.00
        & 0.15 &  0.00 & 0.00
        & 0.20 &  0.00 & 0.00
    \\
\hline[dashed]
CodeGen2
    & Total Prob
        & \textbf{0.09} & \textbf{+0.41} & \textbf{0.02}
        & - & - & -
        & - & - & -
    \\
    & Avg Prob
        & 0.48 & -2.04 & 0.59
        & - & - & -
        & - & - & -
    \\
    & Ask T/F
        & 0.21 & -0.36 & 0.23
        & - & - & -
        & - & - & -
    \\
    & Ask T/F N
        & 0.35 & -1.22 & 0.44
        & - & - & -
        & - & - & -
    \\
    & Verbalize
        & 0.42 & -1.65 & 0.43
        & - & - & -
        & - & - & -
    \\
    & Length
        & 0.51 & -2.21 & 0.60
        & - & - & -
        & - & - & -
    \\
    & Unskilled
        & 0.16 &  0.00 & 0.00
        & - & - & -
        & - & - & -
    \\
\bottomrule
        \end{tblr}
    }
         \caption{\scriptsize Calibration measured as raw, nonscaled Brier Score (${\mathcal B}$), Skill Score ($SS$), and Expected Calibration Error ($ECE$), with respect to ``exact-match'' (EM) notion of correctness, excluding function synthesis tasks as EM is not a useful or commonly used notion of correctness. CodeGen2 repair values are omitted as it does not perform the task with greater than 1\% accuracy.}
         \label{tab:brierExactMatchRaw}
     \vspace*{-2\baselineskip}
\end{table}

==> tables/generated_tables/correctness.tex <==
\begin{tabular}{lrrrr}
\toprule
{} & \multicolumn{2}{l}{Pass@1} & \multicolumn{2}{l}{Exact-Match} \\
Dataset & DyPyBench & DyPyBench-NoDoc &   DyPyBench & DyPyBench-NoDoc \\
Model    &           &                 &             &                 \\
\midrule
CodeGen2 &     28.84 &           23.10 &       19.68 &           15.10 \\
Codex    &     32.96 &           21.69 &       23.60 &           17.77 \\
GPT-3.5  &     33.22 &           26.77 &       23.96 &           18.72 \\
\bottomrule
\end{tabular}


==> tables/generated_tables/dypybench_test_exact_confusion.tex <==
\begin{tabular}{lrrr}
\toprule
Pass@1 &  False &   True &   Total \\
Exact-Match &        &        &         \\
\midrule
False       & 59.89\\% & 16.16\\% &  76.04\\% \\
True        &  6.89\\% & 17.06\\% &  23.96\\% \\
Total       & 66.78\\% & 33.22\\% & 100.00\\% \\
\bottomrule
\end{tabular}


==> tables/generated_tables/performance.tex <==
\begin{tabular}{lrrrlll}
\toprule
{} & \multicolumn{3}{l}{Pass@1} & \multicolumn{3}{l}{Exact-Match} \\
Model & CodeGen2 &  Codex & GPT-3.5 &    CodeGen2 &  Codex & GPT-3.5 \\
Dataset   &          &        &         &             &        &         \\
\midrule
SStubs    &    0.73\\% & 27.77\\% &  20.27\\% &       0.73\\% & 27.77\\% &  20.27\\% \\
DyPyBench &   28.84\\% & 32.96\\% &  33.22\\% &      19.68\\% & 23.60\\% &  23.96\\% \\
Defects4J &    0.00\\% & 23.33\\% &  19.17\\% &       0.00\\% & 19.17\\% &  15.00\\% \\
HumanEval &   23.17\\% & 47.24\\% &  64.60\\% &           - &      - &       - \\
MBPP      &   29.08\\% & 61.79\\% &  72.04\\% &           - &      - &       - \\
\bottomrule
\end{tabular}


==> tables/generated_tables/rocExactMatchRaw.tex <==
% This file was autogenerated by gen_table.py
% SHA 27cfcbd282 - UNCOMMITED CHANGES
% Generate Date UTC 2024-01-23-05-56-31
% It is not recommended to edit this file directly
\definecolor{improvement}{rgb}{1,0,0}
\definecolor{modelrow}{gray}{0.85}

\begin{table}
    \centering
    \resizebox{0.7\columnwidth}{!}{
        \begin{tblr}{
            colspec = {llccccc},
            vline{3,4,6} = {3-24}{gray!75, dotted},
            columns = {font=\small},
                }

            &  & \SetCell[c=1]{c} \textbf{Line Completion} & \SetCell[c=2]{c} \textbf{Function Synthesis} & &
            \SetCell[c=2]{c} \textbf{Program Repair} & \\
            \cmidrule[gray!75]{3} \cmidrule[lr,gray!75]{4-5} \cmidrule[l,gray!75]{6-8}

             Model & Metric & \SetCell[c=1]{c} DyPyBench &
             \SetCell[c=1]{c} HumanEval &
             \SetCell[c=1]{c} MBPP &
             \SetCell[c=1]{c} Defects4J &
             \SetCell[c=1]{c} SStubs \\
            \cmidrule[l]{1-17}
GPT-3.5
    & Total Prob
        & 0.88
        & 0.64
        & 0.61
    \\
    & Avg Prob
        & 0.84
        & 0.64
        & 0.60
    \\
    & Ask T/F
        & 0.49
        & 0.67
        & 0.54
    \\
    & Ask T/F N
        & 0.48
        & 0.70
        & 0.57
    \\
    & Verbalize
        & 0.52
        & 0.51
        & 0.51
    \\
    & Length
        & 0.64
        & 0.50
        & 0.53
    \\
    & Unskilled
        & 0.50
        & 0.50
        & 0.50
    \\
\hline[dashed]
Codex
    & Total Prob
        & 0.90
        & 0.60
        & 0.66
    \\
    & Avg Prob
        & 0.85
        & 0.62
        & 0.65
    \\
    & Ask T/F
        & 0.41
        & 0.61
        & 0.61
    \\
    & Ask T/F N
        & 0.42
        & 0.55
        & 0.59
    \\
    & Verbalize
        & 0.51
        & 0.50
        & 0.49
    \\
    & Length
        & 0.68
        & 0.44
        & 0.49
    \\
    & Unskilled
        & 0.50
        & 0.50
        & 0.50
    \\
\hline[dashed]
CodeGen2
    & Total Prob
        & 0.89
        & -
        & -
    \\
    & Avg Prob
        & 0.82
        & -
        & -
    \\
    & Ask T/F
        & 0.49
        & -
        & -
    \\
    & Ask T/F N
        & 0.53
        & -
        & -
    \\
    & Verbalize
        & 0.50
        & -
        & -
    \\
    & Length
        & 0.68
        & -
        & -
    \\
    & Unskilled
        & 0.50
        & -
        & -
    \\
\hline[dashed]
\bottomrule
        \end{tblr}
    }
         \caption{\scriptsize AUC-ROC score of each technique}
         \label{tab:rocExact MatchRaw}
     \vspace*{-2\baselineskip}
\end{table}
